Generative Adversarial Networks for Automatic Polyp Segmentation

This paper aims to contribute in bench-marking the automatic polyp segmentation problem using generative adversarial networks framework. Perceiving the problem as an image-to-image translation task, conditional generative adversarial networks are utilized to generate masks conditioned by the images as inputs. Both generator and discriminator are convolution neural networks based. The model achieved 0.4382 on Jaccard index and 0.611 as F2 score.

==> takeout.tex <==




% \section{Evaluation Methodology}
% The evaluation methodology for both tasks are as follows:
% \begin{enumerate}
% \item For task 1, we ask the participants to submit the predicted masks in a zip file. The resolution of the predicted mask must be equal to the test images. 
% \item For task 2, the submissions will be verified by inspecting the corresponding docker image.
% \end{enumerate}
%More description about the docker submission, evaluation methodology, evaluation metrics, and challenge design can be found here \footnote{\url{https://github.com/DebeshJha/Medico-automatic-polyp-segmentation-challenge}}.
%The submissions will be verified by inspecting the corresponding docker image. If the participants have problem with submitting the docker image, we are flexible to accept a zip file that contains the predicted mask for\textit{ task 1}.



%\section{Evaluation Metrics and Task}
%\paragraph{\textbf{Automatic polyp segmentation task:}} For the automatic polyp segmentation task, the most commonly used metrics are the Dice similarity coefficient (DSC) or overlap index, and the mean Intersection over Union (mIoU), also known as the Jaccard index.

%The dice similarity coefficient is a metric for comparison of the similarities between two given samples. The DSC is given as
%\begin{equation}\label{eq:dice}
%\text{DSC} = \frac{2 \cdot tp} {2 \cdot tp + fp + fn}
%\end{equation}

%The IoU or JC  is defined as the ratio of intersection of two metrics over a union of two corresponding metrics.  The mean IoU computes IOU of each semantic class of an image and calculate the mean over each classes. The IoU is defined as:

%\begin{equation}\label{eq:iou}
%\text{JC or IoU} = \frac{tp} {tp + fp + fn}
%\end{equation}




%In the polyp image segmentation task (binary segmentation task), precision shows over-segmentation, and recall shows under-segmentation. Thus, we also encourage to calculate precision and recall.


%The precision (positive predictive value) is given by: 

%\begin{equation}
%\text{Precision} =\frac{tp} {tp + fp}
%\end{equation}
%============================================================== 

%and the recall (true positive rate) is given by:
%\begin{equation}
%\text{Recall} = \frac{tp} {tp + fn}.
%\end{equation}

%In the above equations, \textit{tp} represents the true positive, \textit{tn} represents the true negative, \textit{fp} represents the false positive, and \textit{fn} represents the false negative. 

%For \textit{automatic polyp segmentation task}, \textbf{mIoU} is used for evaluation and ranking of the teams. There is a direct correlation between mIoU and DSC. Therefore, we have only used one metric. If the teams have the same mIoU values, then the teams will be further evaluated on the basis of the higher value of the DSC. Moreover, we encourage calculating all the  standard metrics such as DSC, precision, recall, and F2. For the evaluation, we ask the participants to submit the predicted masks in a zip file. The resolution of the predicted mask must be equal to the test images. 

%\paragraph{\textbf{ Algorithm Efficiency Task:}} For the algorithm efficiency task, we require participants to submit their proposed algorithm as part of a Docker image so that we can evaluate it on our hardware. We evaluate the performance on algorithm on Volta 100 GPU, an Nvidia DGX-2 server. Submissions for \textit{algorithm efficiency task} will be evaluated based on the algorithms speed and segmentation performance. The segmentation performance will be measured using the same metrics as described in the \textit{automatic polyp segmentation task} whereas speed will be measured by frames-per-second.

%The speed calculation is calculated as
%\begin{equation}\label{fps}
%\text {Frames Per Second}~(FPS) = {\frac{1} {sec /frame}} = {\frac{\#frames} {sec}}
%\end{equation}

%For this task, we require participants to submit their proposed algorithm as part of a Docker image so that we can evaluate it on our hardware. We evaluate the performance on algorithm on Volta 100 GPU, an Nvidia DGX-2 server.

%Colonoscopy is a standard medical procedure for the examination of colon cancer. 
%Regular screening of such cancer through colonoscopy is a prerequisite for early cancer detection and prevention, and 



%our aim is to provide a formal framework for evaluating the current state of the art, gather researchers in the field and provide high quality data with protocols for validating endoscopic vision algorithms.





%Common datasets and benchmarking of the methods are essential for developing automated semantic segmentation approaches for clinical translation. 

%An automatic polyp detection or surveillance system can help low-cost design solutions and save doctors time, which they could use to look for severe cases. 
%The main objectives of the 2020 Medico Challenge are
%\begin{enumerate}
%\item The challenge offer croudsourcing based opportunity to solve the automatic polyp segmentation task. 
%\item We provide common dataset so that the evaluation of the approaches can be done under same conditions. 
%\end{enumerate}


%Challenges are formal platforms to invite researchers working to address the same problem. By inviting the multiple participants, we provide an opportunity to the researchers to evaluate current state-of-the-art algorithm on the same dataset. Thus, through this year's Medico challenge, we challenge the participants on the Kvasir-SEG dataset to develop more efficient algorithms and solve the polyp segmentation task. 

%is an important step towards designing a system using a high quality dataset, and 

%Moreover, we encourage calculating all the  standard metrics such as DSC, precision, recall, and F2. 


%\textit{tp} represents the true positive, \textit{tn} represents the true negative, \textit{fp} represents the false positive, and \textit{fn} represents the false negative, then the
